$hp$-FEM for the fractional heat equation

We consider a time dependent problem generated by a nonlocal operator in space. Applying a discretization scheme based on $hp$-Finite Elements and a Caffarelli-Silvestre extension we obtain a semidiscrete semigroup. The discretization in time is carried out by using $hp$-Discontinuous Galerkin based timestepping. We prove exponential convergence for such a method in an abstract framework for the discretization in the original domain $\Omega$.

==> figures/contour.tex <==
\begin{tikzpicture}
\fill[fill=blue!10] (-1,-4) -- (2,-4) -- (2,4) -- (-1,4) -- cycle ;
\fill[fill=blue!10] let \p1= (22.5:7) in 
(2,0) -- (22.5:7) -- (\x1,4) -- (2,4) ;

\fill[fill=blue!10] let \p1= (-22.5:7) in
(2,0) -- (-22.5:7) -- (\x1,-4) -- (2,-4) ;


\draw[dashed,fill=white] (0,0) circle (0.5);
\node (eps) at (-0.7,0.1) {$\varepsilon_0$};

\draw[<->] (-1.5,0) -- (6.5,0);
\draw[<->] (0,-4.5) -- (0,4.5);

\draw[thick] (0,0) -- (45:5);
\draw[color=white] (0,0) -- (45:1);

\draw[thick] (0,0) -- (-45:5);
\draw[color=white] (0,0) -- (-45:1);

\node (c) at (1.8,-2.5) {$\mathcal{C}_1$};
\node (c2) at (1.25,0.24) {$\mathcal{C}_2$};
\node (c3) at (1,1.5) {$\mathcal{C}_3$};
\node[font=\huge] (s) at (4,2.5) {$ \mathcal{S}$};



\draw[thick] (0,0) ++(-45:1)  arc (-45:45:1) ;


\draw[dashed] (2,0) -- (22.5:7);
\draw[dashed] (2,0) -- (-22.5:7);
\node (z0) at (2,-0.3) {$z_0$};
\draw[fill,thick] (2,-0.1) -- (2,0.1);


\end{tikzpicture}

==> figures/conv_2d.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{semilogyaxis}[
    width=1.0\textwidth, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$M$: number of layers,
    ylabel= {$L^2(\Omega \times [0,T])$-error},
    legend style={legend pos=south west, legend cell align=left},
    %legend style={at={(0,-0.3)},anchor=north west,legend cell align=left},
    xtick={2,3,4,5,6,7,8,9},
    %xtick=
    %x tick label style={yshift=-0.5em,log x ticks with fixed point},
    %xmax=20000
    ]
      
    % import the correct data from a CSV file
    % condition of not preconditioned
    \addplot+[solid,mark=square,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=L,%x expr=\thisrow{L},
    y=e,
    col sep=comma
    ]{../figures/data/2d/hp.csv};    


    
    \addplot [black,dashed ] expression [domain=2:10, samples=15] { 1.8*2^(-1.5*x)} node [pos=0.6,inner sep=2pt, anchor=south west] {$\bigO(2^{-\frac{3}{2}M})$};

    \legend{$hp-DG$}
  \end{semilogyaxis} 
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../hp_parabolic_frac"
%%% End:


==> figures/conv_u1.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{loglogaxis}[
    width=0.8\textwidth, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$N$: number of systems solved,
    ylabel= {$L^2(\Omega \times [0,T])$-error},
    legend style={legend pos=south west, legend cell align=left},
    %legend style={at={(0,-0.3)},anchor=north west,legend cell align=left},
    xtick={1,10,100,1000},
    %xtick=
    x tick label style={yshift=-0.5em,log x ticks with fixed point},
    xmax=20000
    ]
      
    % import the correct data from a CSV file
    % condition of not preconditioned
    \addplot+[solid,mark=square,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x expr=\thisrow{L}^2,
    y=e,
    col sep=comma
    ]{figures/data/u1/hp.csv};    


    \addplot+[solid,mark=o,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x expr=2^\thisrow{L},
    y=e,
    col sep=comma
    ]{figures/data/u1/uniform.csv};    


    \addplot+[solid,mark=x,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x expr=2^\thisrow{L},
    y=e,
    col sep=comma
    ]{figures/data/u1/graded.csv};    

    
    \addplot [black,dashed ] expression [domain=4:100, samples=15] { 1*2^(-1.25*sqrt(x))} node [pos=1.05,inner sep=2pt, anchor=south west] {$\bigO(2^{-1.25\sqrt{N}})$};
    \addplot [black,dashed ] expression [domain=10:2024, samples=15] { 0.5*x^(-0.75)} node [pos=0.4,inner sep=2pt, anchor=south west] {$\bigO(N^{0.75})$};
    \addplot [black,dashed ] expression [domain=100:2024, samples=15] { 0.81*x^(-1)} node [pos=1.1,inner sep=1pt, anchor=south west] {$\bigO(N^{1})$};


    \legend{$hp-DG$, uniform, graded}
  \end{loglogaxis} 
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../hp_parabolic_frac"
%%% End:


==> figures/conv_ureg.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{semilogyaxis}[
    width=1.0\textwidth, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$M$: number of layers,
    ylabel= {$L^2(\Omega \times [0,T])$-error},
    legend style={legend pos=south west, legend cell align=left},
    %legend style={at={(0,-0.3)},anchor=north west,legend cell align=left},
    xtick={1, 2,3,4,5,6,7,8,9,10,11},
    %xtick=
    %x tick label style={yshift=-0.5em,log x ticks with fixed point},
    %xmax=20000
    ]
      
    % import the correct data from a CSV file
    % condition of not preconditioned
    \addplot+[solid,mark=square,mark size=2pt,mark options={line width=1.0pt}] table    
    [
    x=L,%x expr=\thisrow{L},
    y=e,
    col sep=comma
    ]{figures/data/ureg/hp.csv};    


    
    \addplot [black,dashed ] expression [domain=4:11, samples=15] { 1003.8*2^(-3.5*x)} node [pos=0.6,inner sep=2pt, anchor=south west] {$\bigO(2^{-3 M})$};

    \legend{$hp-DG$}
  \end{semilogyaxis} 
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../hp_parabolic_frac"
%%% End:


==> figures/singular_domain.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{scope}[xscale=-1,yscale=1]

\fill[fill=blue!10] (-1,-4) -- (1,-4) -- (1,4) -- (-1,4) -- cycle ;
\fill[fill=blue!10] let \p1= (22.5:7) in
(1,0) -- (22.5:7) -- (\x1,4) -- (1,4) ;

\fill[fill=blue!10] let \p1= (-22.5:7) in
(1,0) -- (-22.5:7) -- (\x1,-4) -- (1,-4) ;


\draw[dashed,fill=white] (0,0) circle (2);
\node (eps) at (-0.9,-1.3) {$2 z_0$};

\draw[<->] (-1.5,0) -- (6.5,0);
\draw[<->] (0,-4.5) -- (0,4.5);

\draw (0,0) -- (12:7);
\draw (0,0) -- (-12:7);

\draw[thick,blue,,<->] (0,0) ++(-12:5)  arc (-12:12:5) ;                                                                                                                                     
\node[blue] (alpha) at (5.4,0.25) {$2\delta$};


\draw[dashed] (1,0) -- (22.5:7);
\draw[dashed] (1,0) -- (-22.5:7);
\node at (1,-0.5) {$z_0$};
\draw[fill,thick] (1,-0.1) -- (1,0.1);

\node[thick,font=\huge] (xi) at (3,2.2) {$\zeta$};

\end{scope}


\end{tikzpicture}
